Detecting new signals under background mismodelling

Searches for new astrophysical phenomena often involve several sources of non-random uncertainties which can lead to highly misleading results. Among these, model-uncertainty arising from background mismodelling can dramatically compromise the sensitivity of the experiment under study. Specifically, overestimating the background distribution in the signal region increases the chances of missing new physics. Conversely, underestimating the background outside the signal region leads to an artificially enhanced sensitivity and a higher likelihood of claiming false discoveries. The aim of this work is to provide a unified statistical strategy to perform modelling, estimation, inference, and signal characterization under background mismodelling. The method proposed allows to incorporate the (partial) scientific knowledge available on the background distribution and provides a data-updated version of it in a purely nonparametric fashion without requiring the specification of prior distributions on the parameters. Applications in the context of dark matter searches and radio surveys show how the tools presented in this article can be used to incorporate non-stochastic uncertainty due to instrumental noise and to overcome violations of classical distributional assumptions in stacking experiments.

==> Extra_text.tex <==

Let $\bm{x}=(x_{1},\dots,x_{n})$ be a data sample  on which we would like to assess whether the signal of interest is present or not.  Suppose that, in addition to 
$\bm{x}$,  a  source-free  dataset  $\tilde{\bm{x}}=(\tilde{x}_{1},\dots,\tilde{x}_{N})$ is given. The latter may be a sample of observations   from control regions or the result of Monte Carlo simulations,  assuming that no signal is present. 
Hereafter,  refer to $\bm{x}$ as the \emph{physics sample} and to $\tilde{\bm{x}}$ as the \emph{source-free sample}. Notice that, if no source is present, both $\tilde{\bm{x}}$ and $\bm{x}$ are distributed according to $f_b(x)$. Therefore,
 $\tilde{\bm{x}}$  can be used to ``learn'' the unknown pdf of the background, namely $f_b(x)$.  
 
  Despite my future research does involve extensions to the discrete setting, there are a few reason why in my article I have decided to limit the attention to the continuous setting. First of all,  the constructs involved are easier  to understand for the continuous case rather than the general continuous/discrete setting and I believe this should be the place to start as a first exposure to LP modelling. Second, the confidence bands in (25) can only be constructed  via tube formulae for the continuous case. Third, even if I was to consider also the discrete case, the underlying assumption here is that the observations are i.i.d whereas, for my understanding of the most standard problem in particle physics, the expected number of Poisson events over the energy spectrum for instance varies hence the observations are not identically distributed.
Despite I have recently found a solution for this problem, it would require the introduction of additional constructs and additional methods and thus 

The estimate $\widehat{d}(u;G,F)$ in \eqref{dhat} can equivalenty be rewritten as
\[\widehat{d}(u;G,F)=\sum_{j=0}^M<Leg_j(u),\tilde{d}(u)>Leg_j(u)\]
where $\tilde{d}(u)$ denotes the empirical pdf of the sample $u_1,dots,u_n$. Therefore,  when $M=n-1$,
 $\widehat{d}(u;G,F)$ is equal to $\tilde{d}(u)$ and, because of \eqref{fhat}, $\widehat{f}(x)\equiv\tilde{f}(x)$
 at points $x_1,\dots,x_n$. It follows from \eqref{MSE} that, when $M<n-1$ the estimators in \eqref{dhat} and \eqref{fhat} will exhibit  lower variance and higher variance than the classical sample estimators.



\begin{array}
\label{bias}
\text{bias}\bigl[\widehat{d}(u;G,F)\bigl]&=E\bigl[\widehat{d}(u;G,F)\bigl]-d(u;G,F)\\
 &=
\end{array}
 
 
 Furthermore, it can be shown \cite{LPmode} that, as $n\rightarrow\infty$
\begin{equation}
\label{lpH0}
\sqrt{n}\widehat{LP}_j\xrightarrow{d} N(0, 1),
\end{equation} 
where $\xrightarrow{d}$ denotes convergence in distribution. 

\begin{equation}
\begin{split}
\label{MSE}
MSE\Bigl[\widehat{d}(u;G,F)\Bigl]&=E\biggl[\bigl(\widehat{d}(u;G,F)-d(u;G,F)\bigl)^2\biggl]\\
&=\text{Bias}^2\bigl[\widehat{d}(u;G,F)\bigl]+V\bigl[\widehat{d}(u;G,F)\bigl]
\end{split}
\end{equation}
where, as shown in Appendix \ref{appB}, $\text{Bias}\bigl[\widehat{d}(u;G,F)\bigl]$ and $V\bigl[\widehat{d}(u;G,F)\bigl]$ are given by
\begin{align}
\label{bias}
\text{Bias}\bigl[\widehat{d}(u;G,F)\bigl]&=\sum_{j>M}LP_jLeg_j(u)\qquad \text{and}\\
\label{variancedhat}
V\bigl[\widehat{d}(u;G,F)\bigl]&=\sum_{j=1}^{M}\frac{\sigma^2_j}{n}Leg^2_j(u)+2\sum_{j<k}\frac{\sigma_{jk}}{n}Leg_j(u)Leg_k(u).
\end{align}
Conversely, the bias is only affected by the number of terms contributing to the sum in \eqref{dhat} and thus it decreases as $M$ increases.}

\red{Despite the above definitions are only pointwise,  it is possible to assess the bias and 
the risk over the unit inval by considering the mean integrated squared error (MISE) i.e.,

 \red{The sample dsitribution function  is
\begin{equation}
\label{ecdf}
\tilde{F}(x)=\frac{1}{n}\sum_{i=1}^n \mathbb{1}_{x_i<x},
\end{equation}
